Stealthy Attack on Algorithmic-Protected DNNs via Smart Bit Flipping

Recently, deep neural networks (DNNs) have been deployed in safety-critical systems such as autonomous vehicles and medical devices. Shortly after that, the vulnerability of DNNs were revealed by stealthy adversarial examples where crafted inputs -- by adding tiny perturbations to original inputs -- can lead a DNN to generate misclassification outputs. To improve the robustness of DNNs, some algorithmic-based countermeasures against adversarial examples have been introduced thereafter. In this paper, we propose a new type of stealthy attack on protected DNNs to circumvent the algorithmic defenses: via smart bit flipping in DNN weights, we can reserve the classification accuracy for clean inputs but misclassify crafted inputs even with algorithmic countermeasures. To fool protected DNNs in a stealthy way, we introduce a novel method to efficiently find their most vulnerable weights and flip those bits in hardware. Experimental results show that we can successfully apply our stealthy attack against state-of-the-art algorithmic-protected DNNs.

==> Back.tex <==
% 1)The attacker is co-located with the victim DNN service, and can run user-space unprivileged processes.
% 2)Additionally, it can map pages in the weight file to its own address space in read-only mode. To map virtual address to physical address, the attacker can take advantage of huge page support. If such support is not available in the system, the attacker can leverage hardware-based side channels [] or use advanced memory massaging techniques [].

We mainly harness double-sided rowhammer technique as it has been shown to be most effective in inducing bit flips. Double-sided rowhammer relies on a settlement of two adjacent rows to the victim row, and thus requires knowledge of DRAM addressing scheme, which could be obtained through reverse engineering

In particular, [X] show that by abusing Linux’ memory deduplication system (KSM) [6] which is very popular in production clouds [8], and the widespread Rowhammer DRAM bug [34], an attacker can reliably flip a single bit in any physical page in the software stack with known contents.

Errors are data-pattern dependent. The Solid data-pattern (all ‘0’s or all ‘1’s) yields the fewest errors, whereas the Row Stripe data-pattern (alternating rows of ‘0’s and ‘1’s) yields the most errors.

The attacker needs to control the bit flips precisely at the targeted locations since extra bit flips undermine the effectiveness of our attack.
Therefore, the attacker should avoid simultaneous bit flip at undesired page offsets.
[] designs a precise rowhammering technique using a new data pattern called column-page-stripe data pattern.

A row-hammer attack [] on Dynamic Random Access Memory (DRAM) is the most popular one since it can create a profile of memory bits stored inside the main memory (i.e., DRAM) and flip any bit of a given target address.

Second, to understand the practical impact of this vulnerability, we use Rowhammer [26] as an exemplary hardware fault attack. While a variety of hardware fault attacks are documented in literature [11, 26, 38, 57], Rowhammer is particularly amenable to practical, real-world exploitation. Rowhammer takes advantage of a widespread vulnerability in modern DRAM modules and provides an attacker with the ability to trigger controlled memory corruptions directly from unprivileged software execution. As a result, even a constrained Rowhammer-enabled attacker, who only needs to perform a specific memory access pattern, can mount practical attacks in a variety of real-world environments, including cloud [44,67], browsers [9, 15, 19, 48], mobile [15, 62], and servers [36, 60].

Our Rowhammer results show that in a surgical attack scenario, with the capability of flipping specific bits, the attacker can reliably cause severe accuracy drops in practical settings.

Rowhammer is the most common instance of software-induced fault attacks [9, 15, 19, 44, 48, 60, 62, 67]. This vulnerability provides an aggressor with a single-bit corruption primitive at DRAM level; thus, it is an ideal attack for the purpose of our analysis. Rowhammer is a remarkably versatile fault attack since it only requires an attacker to be able to access content in DRAM; an ubiquitous feature of every modern system. By simply carrying out specific memory access patterns—which we explain in Sec 5—the attacker is able to cause extreme stress on other memory locations triggering faults on other stored data.


Victor van der Veen, Yanick Fratantonio, Martina Lindorfer, Daniel Gruss, Clementine Maurice, Giovanni Vigna, Herbert Bos, Kaveh Razavi, and Cristiano Giuffrida. 2016. Drammer: Deterministic Rowhammer Attacks on Mobile Platforms. In Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security (CCS '16). Association for Computing Machinery, New York, NY, USA, 1675–1689. DOI:https://doi.org/10.1145/2976749.2978406

Kim, Jeremie S., et al. "Revisiting rowhammer: An experimental analysis of modern dram devices and mitigation techniques." 2020 ACM/IEEE 47th Annual International Symposium on Computer Architecture (ISCA). IEEE, 2020.

[1] Kaveh Razavi, Ben Gras, Erik Bosman, Bart Preneel, Cristiano Giuffrida, and Herbert Bos. Flip feng shui: Hammering a needle in the software stack. In 25th USENIX Security Symposium (USENIX Security 16), pages 1–18, Austin, TX, 2016. USENIX Association.

[2] Victor Van Der Veen, Yanick Fratantonio, Martina Lindorfer, Daniel Gruss, Clémentine Maurice, Giovanni Vigna, Herbert Bos, Kaveh Razavi, and Cristiano Giuffrida. Drammer: Deterministic rowhammer
attacks on mobile platforms. In Proceedings of the 2016 ACM SIGSAC conference on computer and communications security, pages 1675–1689. ACM, 2016.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

However, recent works have demonstrated that bit flips are still possible even with the presence of such hardware-based protections [].
